Approaching the Source of Symbol Grounding with Confluent Reductions of Abstract Meaning Representation Directed Graphs

Abstract meaning representation (AMR) is a semantic formalism used to represent the meaning of sentences as directed acyclic graphs. In this paper, we describe how real digital dictionaries can be embedded into AMR directed graphs (digraphs), using state-of-the-art pre-trained large language models. Then, we reduce those graphs in a confluent manner, i.e. with transformations that preserve their circuit space. Finally, the properties of these reduces digraphs are analyzed and discussed in relation to the symbol grounding problem.

==> latex/algorithms/confluent_reduction.tex <==
\begin{algorithm}
  \caption{Reduce a directed graph confluently}\label{algo:reduce-conf}
  \begin{algorithmic}[1]
    \Function{ReduceConfluent}{$G$ : digraph}
      \Repeat
        \Repeat \Comment{Apply cheap reductions first}
          \State $G' = G$
          \State $G' \gets \Loop(G')$
          \State $G' \gets \Subset(G')$
          \State $G' \gets \Indiclique(G')$
          \State $G' \gets \Outdiclique(G')$
        \Until{$G = G'$}
        \State $G' = G$ \Comment{Apply costly reduction}
        \State $G' \gets \Pie(G')$
      \Until{$G = G'$}
      \State \Return $G$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> latex/algorithms/save_AMRs.tex <==
\begin{algorithm}
    \caption{Minimize invalid AMRs quantity}\label{algo:min-amr}
    \begin{algorithmic}[1]
        \Function{SaveAMRs}{$invalid\_AMRs$ : list}
        \EndFunction
    \end{algorithmic}
\end{algorithm}

==> latex/r__ponse.tex <==
1. Before specifically addressing the content of this point, we want to specify we are not studying meaning representations in LLMs nor are we trying to make hypotheses about how meaning is represented in modern AI models. We used a pre-trained transformer model to generate the AMR graphs, not as a scientific position but simply as a \textit{tool}. We are reporting empirical findings on dictionaries. 

Our position is that the Symbol Grounding Problem remains an open one and that we are simply making a tiny step in the direction of studying \textit{grounding sets}. We are not (yet) interested in proposing a model through this work.

Regarding the first half of your comment, we are not sure what is meant by the following and would gladly appreciate a further clarification : 

```
This paper reifies word definitions in the way it formalises the symbol grounding problem. This is, I would say, a view well outside the mainstream of cognitive science/linguistics, where it is widely accepted that necessary and sufficient conditions are not a tenable way of describing word usage.
```

We must mention we are not pretending to model the Symbol Grounding Problem itself, we are trying to approach it by approximation. The problem of identifying the smallest number of words that needs to be known in order to learn all other in a dictionary is different than the problem of identifying the smallest number of words that needs to be known before an actual human can learn all other words, which itself is different from the Symbol Grounding Problem as originally coined by Stevan Harnad : explaining how and why humans have the unique capacity to ground arbitrary symbols in the things in the world they refer to.

We are also not proposing a model of definition and language learning in humans but we are indeed stating that languages cannot be learned via definition (verbal instructions) alone. 

While we are not sure what is meant, we wish to say the following in response : 

(a) Neither sensorimotor learning of categories nor verbal definition of categories is based on a notion of necessary and sufficient conditions.

(b) To categorize is to do the right thing with the right kind of thing: Eat what’s edible and not what is toxic; call cats “cats” and dogs “dogs” and catastrophes “catastrophes”. Approach cats and dogs but not catastrophes.

(c) Learning to do the right thing with the right kind of thing is based on supervised (reinforcement) learning: trial and error with corrective feedback from the consequences of doing the right thing or the wrong thing.

(d) No set of features of features is necessary/sufficient and exhaustive in the real world of human category learning. All categories, hence features, are approximate and provisional. It is only in the formal world of mathematics and logic that necessary and sufficient conditions can be provided by formal definition and formal proof: An “even number” is an integer divisible by 2.

(e) The dictionary definition of the referent of a content-word (which is always the name of a category) is not true by formal definition and proof, as in maths: “A cat has pointy ears and purrs” may be enough to sort cats and dogs for a few instances, but it remains approximate and provisional, since there is an infinite number of possible inputs. The definition can be extended and tightened, but it is never provably exhaustive, necessary or sufficient.

2. We agree with you that the motivations should explained more clearly, as our positions, rather than assumed. This was done because we are continuing from an already going body of work and due to space constraints. We are not making comments about the processes going on in the brain nor are we proposing a model that would work using this constrained set. 

Here is our position regarding our cognitive model. The cognitive model of the lexicon in the head of a grounded categorizer and language-user is based on the hypotheses that categories can be learned indirectly through definition alone based on a dictionary’s MinSet (or an LM, or a teacher) as long as the MinSet is grounded in the head of the human learner by prior direct sensorimotor category learning. The direct sensorimotor (i.e., perceptual) grounding of at least one MinSet is the source of the “psychological” reality.

3. Due to the short time we have to reply to this point, we cannot provide new results or examples. However, we appreciate these points and we will take them into account as we further refine the paper. 

4. We whole-heartedly agree with you that Symbol Grounding is a problem for humans and not English speakers only. This focus on English is only due to the fact that we only had access to English dictionaries we could use (at the time of writing, as we have since started analyzing two french dictionaries). It was a mistake on our end to not address this in the limitations. We also hope to extend our approach to dictionaries of other languages by using BabelNet-Meaning-Representation. 

We agree with all your comment suggestions and will make the necessary changes. We lacked rigor when referring to concepts such word or symbol and will fix these incorrect isomorphism. 

Overall we appreciate your comments and believe it will help us refine this paper. 

==> latex/r__ponse_2.tex <==
We want to begin by stating that we agree with your suggestions regarding the needed clarifications about our emphasis on the *Symbol Grounding Problem* (SGP), which we maintain is the theoretical (and empirical) motivation for this work. In that regards, considering reviewer 1 expressed similar concerns, we are committed to re-drafting certain sections and moving some of the graph theoretical notations to the appendix within this cycle, as to leave more space for these clarifications. However we would also like to clarify our theoretical position within the context of this back-and-forth, especially to address this point : 

```
So that aspect needs clarification: if there is no grounding, what's the relevance to the symbol grounding problem?
```











%We want to begin by stating that we agree with you that there are improvements and clarifications needed regarding our motivations and our emphasis on the *Symbol Grounding Problem* and the related issue of identifying minimal grounding sets (in a dictionary) as it is *indeed* our main motivation. 

==> latex/tables/3_types_graph_confl.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|lll|lll|lll|lll|lll|lll|lll|lll|}
\hline
           & \multicolumn{3}{c|}{WordNet}                                      & \multicolumn{3}{c|}{MerWeb}                                      & \multicolumn{3}{c|}{WEDT}                                          & \multicolumn{3}{c|}{LDOCE}                                         & \multicolumn{3}{c|}{CIDE}                                          & \multicolumn{3}{c|}{WCDT}                                        & \multicolumn{3}{c|}{WLDT}                                       & \multicolumn{3}{c|}{WILD}                                       \\ \hline
Nb Remain. & \multicolumn{1}{l|}{2 068}   & \multicolumn{1}{l|}{TODO} & 6 485  & \multicolumn{1}{l|}{1 968}  & \multicolumn{1}{l|}{TODO} & 6 670  & \multicolumn{1}{l|}{1 601}  & \multicolumn{1}{l|}{4 833}  & 3 886  & \multicolumn{1}{l|}{436}    & \multicolumn{1}{l|}{2 031}  & 1 744  & \multicolumn{1}{l|}{696}    & \multicolumn{1}{l|}{1 719}  & 1 486  & \multicolumn{1}{l|}{389}    & \multicolumn{1}{l|}{1 222} & 948   & \multicolumn{1}{l|}{151}   & \multicolumn{1}{l|}{300}   & 291   & \multicolumn{1}{l|}{408}   & \multicolumn{1}{l|}{0}     & 239   \\ \hline
Nb Incl.   & \multicolumn{1}{l|}{548}     & \multicolumn{1}{l|}{}     & 7 252  & \multicolumn{1}{l|}{1 125}  & \multicolumn{1}{l|}{}     & 8 631  & \multicolumn{1}{l|}{899}    & \multicolumn{1}{l|}{6 383}  & 5 874  & \multicolumn{1}{l|}{390}    & \multicolumn{1}{l|}{2 074}  & 2 226  & \multicolumn{1}{l|}{185}    & \multicolumn{1}{l|}{2 030}  & 2 102  & \multicolumn{1}{l|}{460}    & \multicolumn{1}{l|}{1 801} & 1 906 & \multicolumn{1}{l|}{208}   & \multicolumn{1}{l|}{780}   & 807   & \multicolumn{1}{l|}{172}   & \multicolumn{1}{l|}{678}   & 528   \\ \hline
Nb Excl.   & \multicolumn{1}{l|}{143 882} & \multicolumn{1}{l|}{}     & 40 844 & \multicolumn{1}{l|}{94 402} & \multicolumn{1}{l|}{}     & 44 562 & \multicolumn{1}{l|}{50 065} & \multicolumn{1}{l|}{20 042} & 24 223 & \multicolumn{1}{l|}{34 773} & \multicolumn{1}{l|}{16 497} & 18 682 & \multicolumn{1}{l|}{20 214} & \multicolumn{1}{l|}{13 960} & 15 787 & \multicolumn{1}{l|}{11 530} & \multicolumn{1}{l|}{7 384} & 8 075 & \multicolumn{1}{l|}{4 149} & \multicolumn{1}{l|}{3 405} & 3 484 & \multicolumn{1}{l|}{2 633} & \multicolumn{1}{l|}{2 305} & 2 364 \\ \hline
Nb Reduc   & \multicolumn{1}{l|}{5 120}   & \multicolumn{1}{l|}{}     & 6 485  & \multicolumn{1}{l|}{7 079}  & \multicolumn{1}{l|}{}     & 7 543  & \multicolumn{1}{l|}{5 289}  & \multicolumn{1}{l|}{5 172}  & 4 671  & \multicolumn{1}{l|}{1 576}  & \multicolumn{1}{l|}{2121}   & 2 275  & \multicolumn{1}{l|}{1 055}  & \multicolumn{1}{l|}{1 767}  & 1 433  & \multicolumn{1}{l|}{2 531}  & \multicolumn{1}{l|}{1 963} & 2 005 & \multicolumn{1}{l|}{965}   & \multicolumn{1}{l|}{856}   & 910   & \multicolumn{1}{l|}{982}   & \multicolumn{1}{l|}{587}   & 737   \\ \hline
Nb LOOP    & \multicolumn{1}{l|}{409}     & \multicolumn{1}{l|}{}     & 450    & \multicolumn{1}{l|}{818}    & \multicolumn{1}{l|}{}     & 634    & \multicolumn{1}{l|}{814}    & \multicolumn{1}{l|}{461}    & 499    & \multicolumn{1}{l|}{341}    & \multicolumn{1}{l|}{239}    & 228    & \multicolumn{1}{l|}{162}    & \multicolumn{1}{l|}{130}    & 135    & \multicolumn{1}{l|}{415}    & \multicolumn{1}{l|}{257}   & 278   & \multicolumn{1}{l|}{185}   & \multicolumn{1}{l|}{153}   & 146   & \multicolumn{1}{l|}{160}   & \multicolumn{1}{l|}{96}    & 74    \\ \hline
Nb SUBSET  & \multicolumn{1}{l|}{3}       & \multicolumn{1}{l|}{}     & 5      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{}     & 3      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{4}      & 3      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & 1      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{0}      & 0      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{3}     & 1     & \multicolumn{1}{l|}{1}     & \multicolumn{1}{l|}{1}     & 1     & \multicolumn{1}{l|}{1}     & \multicolumn{1}{l|}{0}     & 0     \\ \hline
Nb IN      & \multicolumn{1}{l|}{431}     & \multicolumn{1}{l|}{}     & 361    & \multicolumn{1}{l|}{924}    & \multicolumn{1}{l|}{}     & 856    & \multicolumn{1}{l|}{427}    & \multicolumn{1}{l|}{291}    & 297    & \multicolumn{1}{l|}{199}    & \multicolumn{1}{l|}{67}     & 81     & \multicolumn{1}{l|}{113}    & \multicolumn{1}{l|}{54}     & 61     & \multicolumn{1}{l|}{374}    & \multicolumn{1}{l|}{158}   & 179   & \multicolumn{1}{l|}{193}   & \multicolumn{1}{l|}{97}    & 100   & \multicolumn{1}{l|}{126}   & \multicolumn{1}{l|}{160}   & 50    \\ \hline
Nb OUT     & \multicolumn{1}{l|}{4 084}   & \multicolumn{1}{l|}{}     & 4 981  & \multicolumn{1}{l|}{5 051}  & \multicolumn{1}{l|}{}     & 5 686  & \multicolumn{1}{l|}{3 763}  & \multicolumn{1}{l|}{4 071}  & 3 560  & \multicolumn{1}{l|}{963}    & \multicolumn{1}{l|}{1 720}  & 1 913  & \multicolumn{1}{l|}{717}    & \multicolumn{1}{l|}{1 351}  & 1 205  & \multicolumn{1}{l|}{1 477}  & \multicolumn{1}{l|}{1 487} & 1 461 & \multicolumn{1}{l|}{550}   & \multicolumn{1}{l|}{600}   & 603   & \multicolumn{1}{l|}{585}   & \multicolumn{1}{l|}{331}   & 436   \\ \hline
Nb PIE     & \multicolumn{1}{l|}{193}     & \multicolumn{1}{l|}{}     & 1 163  & \multicolumn{1}{l|}{284}    & \multicolumn{1}{l|}{}     & 364    & \multicolumn{1}{l|}{282}    & \multicolumn{1}{l|}{345}    & 312    & \multicolumn{1}{l|}{70}     & \multicolumn{1}{l|}{94}     & 52     & \multicolumn{1}{l|}{61}     & \multicolumn{1}{l|}{232}    & 32     & \multicolumn{1}{l|}{259}    & \multicolumn{1}{l|}{58}    & 86    & \multicolumn{1}{l|}{36}    & \multicolumn{1}{l|}{5}     & 60    & \multicolumn{1}{l|}{110}   & \multicolumn{1}{l|}{0}     & 177   \\ \hline
\end{tabular}
\end{table}


==> latex/tables/3_types_metrics.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|lll|lll|lll|lll|lll|lll|lll|lll|}
\hline
               & \multicolumn{3}{c|}{WordNet}                                       & \multicolumn{3}{c|}{MerWeb}                                        & \multicolumn{3}{c|}{WEDT}                                             & \multicolumn{3}{c|}{LDOCE}                                            & \multicolumn{3}{c|}{CIDE}                                             & \multicolumn{3}{c|}{WCDT}                                          & \multicolumn{3}{c|}{WLDT}                                          & \multicolumn{3}{c|}{WILD}                                          \\ \hline
Nb vertices    & \multicolumn{1}{l|}{146 498} & \multicolumn{1}{l|}{TODO} & 54 581  & \multicolumn{1}{l|}{97 945}  & \multicolumn{1}{l|}{TODO} & 61 863  & \multicolumn{1}{l|}{52 565}  & \multicolumn{1}{l|}{31 258}  & 33 983  & \multicolumn{1}{l|}{21 095}  & \multicolumn{1}{l|}{20 602}  & 22 652  & \multicolumn{1}{l|}{35 599}  & \multicolumn{1}{l|}{17 709}  & 19 375  & \multicolumn{1}{l|}{3 213}  & \multicolumn{1}{l|}{10 407} & 10 929 & \multicolumn{1}{l|}{12 379} & \multicolumn{1}{l|}{4 485}  & 4 582  & \multicolumn{1}{l|}{4 508}  & \multicolumn{1}{l|}{2 983}  & 3 131  \\ \hline
Size Kernel    & \multicolumn{1}{l|}{7 131}   & \multicolumn{1}{l|}{}     & 19 079  & \multicolumn{1}{l|}{9 070}   & \multicolumn{1}{l|}{}     & 21 843  & \multicolumn{1}{l|}{6 694}   & \multicolumn{1}{l|}{15 578}  & 13 617  & \multicolumn{1}{l|}{1 711}   & \multicolumn{1}{l|}{5 892}   & 5 964   & \multicolumn{1}{l|}{1 988}   & \multicolumn{1}{l|}{5 154}   & 4 854   & \multicolumn{1}{l|}{1 291}  & \multicolumn{1}{l|}{4 668}  & 4 495  & \multicolumn{1}{l|}{2 183}  & \multicolumn{1}{l|}{1 777}  & 1 801  & \multicolumn{1}{l|}{1 103}  & \multicolumn{1}{l|}{1 169}  & 1 253  \\ \hline
Size Red. Ker. & \multicolumn{1}{l|}{2 068}   & \multicolumn{1}{l|}{}     & 6 485   & \multicolumn{1}{l|}{1 968}   & \multicolumn{1}{l|}{}     & 6 670   & \multicolumn{1}{l|}{1 601}   & \multicolumn{1}{l|}{4 833}   & 3 886   & \multicolumn{1}{l|}{696}     & \multicolumn{1}{l|}{2 031}   & 1744    & \multicolumn{1}{l|}{436}     & \multicolumn{1}{l|}{1 719}   & 1 486   & \multicolumn{1}{l|}{408}    & \multicolumn{1}{l|}{1 222}  & 948    & \multicolumn{1}{l|}{389}    & \multicolumn{1}{l|}{300}    & 291    & \multicolumn{1}{l|}{147}    & \multicolumn{1}{l|}{0}      & 239    \\ \hline
NC Red Ker.    & \multicolumn{1}{l|}{2 028}   & \multicolumn{1}{l|}{}     & 6 428   & \multicolumn{1}{l|}{1 933}   & \multicolumn{1}{l|}{}     & 6 541   & \multicolumn{1}{l|}{1 556}   & \multicolumn{1}{l|}{4 785}   & 3 858   & \multicolumn{1}{l|}{683}     & \multicolumn{1}{l|}{2 021}   & 1 738   & \multicolumn{1}{l|}{423}     & \multicolumn{1}{l|}{1 711}   & 1 482   & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{1 191}  & 935    & \multicolumn{1}{l|}{342}    & \multicolumn{1}{l|}{283}    & 272    & \multicolumn{1}{l|}{123}    & \multicolumn{1}{l|}{0}      & 192    \\ \hline
Init. Nb Arcs  & \multicolumn{1}{l|}{765 481} & \multicolumn{1}{l|}{}     & 443 649 & \multicolumn{1}{l|}{495 385} & \multicolumn{1}{l|}{}     & 468 711 & \multicolumn{1}{l|}{273 432} & \multicolumn{1}{l|}{263 966} & 250 349 & \multicolumn{1}{l|}{107 638} & \multicolumn{1}{l|}{202 771} & 194 271 & \multicolumn{1}{l|}{173 737} & \multicolumn{1}{l|}{164 304} & 167 147 & \multicolumn{1}{l|}{22 667} & \multicolumn{1}{l|}{68 043} & 66 999 & \multicolumn{1}{l|}{61 282} & \multicolumn{1}{l|}{25 324} & 24 861 & \multicolumn{1}{l|}{19 133} & \multicolumn{1}{l|}{15 597} & 17 654 \\ \hline
Final Nb Arcs  & \multicolumn{1}{l|}{14 858}  & \multicolumn{1}{l|}{}     & 121 625 & \multicolumn{1}{l|}{14 278}  & \multicolumn{1}{l|}{}     & 122 068 & \multicolumn{1}{l|}{11 109}  & \multicolumn{1}{l|}{82 423}  & 57 671  & \multicolumn{1}{l|}{4 837}   & \multicolumn{1}{l|}{42 883}  & 29 828  & \multicolumn{1}{l|}{2 700}   & \multicolumn{1}{l|}{28 689}  & 22 261  & \multicolumn{1}{l|}{2 860}  & \multicolumn{1}{l|}{12 487} & 9 129  & \multicolumn{1}{l|}{2 524}  & \multicolumn{1}{l|}{2 718}  & 2 566  & \multicolumn{1}{l|}{833}    & \multicolumn{1}{l|}{678}    & 1 910  \\ \hline
NC Final Arcs  & \multicolumn{1}{l|}{14 430}  & \multicolumn{1}{l|}{}     & 117 679 & \multicolumn{1}{l|}{13 831}  & \multicolumn{1}{l|}{}     & 119 414 & \multicolumn{1}{l|}{10 520}  & \multicolumn{1}{l|}{80 898}  & 56 856  & \multicolumn{1}{l|}{4 697}   & \multicolumn{1}{l|}{41 624}  & 29 343  & \multicolumn{1}{l|}{2 539}   & \multicolumn{1}{l|}{27 787}  & 21 894  & \multicolumn{1}{l|}{2 664}  & \multicolumn{1}{l|}{11 934} & 8 815  & \multicolumn{1}{l|}{2 177}  & \multicolumn{1}{l|}{2 523}  & 2 344  & \multicolumn{1}{l|}{703}    & \multicolumn{1}{l|}{0}      & 1 576  \\ \hline
Nb Undefined   & \multicolumn{1}{l|}{144}     & \multicolumn{1}{l|}{}     & 6 824   & \multicolumn{1}{l|}{328}     & \multicolumn{1}{l|}{}     & 8 071   & \multicolumn{1}{l|}{89}      & \multicolumn{1}{l|}{5 950}   & 5 409   & \multicolumn{1}{l|}{22}      & \multicolumn{1}{l|}{1 838}   & 2 002   & \multicolumn{1}{l|}{46}      & \multicolumn{1}{l|}{1 904}   & 1 969   & \multicolumn{1}{l|}{11}     & \multicolumn{1}{l|}{1 545}  & 1 635  & \multicolumn{1}{l|}{48}     & \multicolumn{1}{l|}{632}    & 669    & \multicolumn{1}{l|}{33}     & \multicolumn{1}{l|}{615}    & 454    \\ \hline
Nb Undefining  & \multicolumn{1}{l|}{137 815} & \multicolumn{1}{l|}{}     & 35 257  & \multicolumn{1}{l|}{86 374}  & \multicolumn{1}{l|}{}     & 39 126  & \multicolumn{1}{l|}{44 280}  & \multicolumn{1}{l|}{15 092}  & 20 153  & \multicolumn{1}{l|}{18 843}  & \multicolumn{1}{l|}{14 509}  & 16 599  & \multicolumn{1}{l|}{33 246}  & \multicolumn{1}{l|}{12 319}  & 14 400  & \multicolumn{1}{l|}{1 874}  & \multicolumn{1}{l|}{5 654}  & 6 410  & \multicolumn{1}{l|}{9 278}  & \multicolumn{1}{l|}{2 683}  & 2 764  & \multicolumn{1}{l|}{3 261}  & \multicolumn{1}{l|}{1 751}  & 1 872  \\ \hline
Nb SCCs Kernel & \multicolumn{1}{l|}{253}     & \multicolumn{1}{l|}{}     & 31      & \multicolumn{1}{l|}{459}     & \multicolumn{1}{l|}{}     & 107     & \multicolumn{1}{l|}{385}     & \multicolumn{1}{l|}{32}      & 60      & \multicolumn{1}{l|}{65}      & \multicolumn{1}{l|}{49}      & 58      & \multicolumn{1}{l|}{168}     & \multicolumn{1}{l|}{18}      & 18      & \multicolumn{1}{l|}{18}     & \multicolumn{1}{l|}{31}     & 49     & \multicolumn{1}{l|}{125}    & \multicolumn{1}{l|}{19}     & 15     & \multicolumn{1}{l|}{49}     & \multicolumn{1}{l|}{15}     & 25     \\ \hline
\end{tabular}
\end{table}


==> latex/tables/Old/two_graph_metrics.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
               & \multicolumn{2}{c|}{WordNet}           & \multicolumn{2}{c|}{MerWeb}            & \multicolumn{2}{c|}{WEDT}              & \multicolumn{2}{c|}{LDOCE}             & \multicolumn{2}{c|}{CIDE}              & \multicolumn{2}{c|}{WCDT}            & \multicolumn{2}{c|}{WLDT}            & \multicolumn{2}{c|}{WILD}            \\ \hline
Nb vertices    & \multicolumn{1}{l|}{146 498} & 54 581  & \multicolumn{1}{l|}{97 495}  & 61 863  & \multicolumn{1}{l|}{52 565}  & 33 983  & \multicolumn{1}{l|}{35 599}  & 22 652  & \multicolumn{1}{l|}{21 095}  & 19 375  & \multicolumn{1}{l|}{12 379} & 10 929 & \multicolumn{1}{l|}{4 508}  & 4 582  & \multicolumn{1}{l|}{3 213}  & 3 131  \\ \hline
Size Kernel    & \multicolumn{1}{l|}{7 131}   & 19 079  & \multicolumn{1}{l|}{9 070}   & 21 843  & \multicolumn{1}{l|}{6 694}   & 13 617  & \multicolumn{1}{l|}{1 988}   & 5 964   & \multicolumn{1}{l|}{1 711}   & 4 854   & \multicolumn{1}{l|}{2 813}  & 4 495  & \multicolumn{1}{l|}{1 103}  & 1 801  & \multicolumn{1}{l|}{1 291}  & 1 253  \\ \hline
Size Red. Ker. & \multicolumn{1}{l|}{2 068}   & 6 485   & \multicolumn{1}{l|}{1 968}   & 6 670   & \multicolumn{1}{l|}{1 601}   & 3 886   & \multicolumn{1}{l|}{436}     & 1744    & \multicolumn{1}{l|}{696}     & 1 486   & \multicolumn{1}{l|}{389}    & 948    & \multicolumn{1}{l|}{147}    & 291    & \multicolumn{1}{l|}{408}    & 239    \\ \hline
NC Red Ker.    & \multicolumn{1}{l|}{2 028}   & 6 428   & \multicolumn{1}{l|}{1 933}   & 6 541   & \multicolumn{1}{l|}{1 556}   & 3 858   & \multicolumn{1}{l|}{423}     & 1 738   & \multicolumn{1}{l|}{683}     & 1 482   & \multicolumn{1}{l|}{342}    & 935    & \multicolumn{1}{l|}{123}    & 272    & \multicolumn{1}{l|}{398}    & 192    \\ \hline
Init. Nb Arcs  & \multicolumn{1}{l|}{765 481} & 443 649 & \multicolumn{1}{l|}{495 385} & 468 711 & \multicolumn{1}{l|}{273 432} & 250 349 & \multicolumn{1}{l|}{173 737} & 194 271 & \multicolumn{1}{l|}{107 638} & 167 147 & \multicolumn{1}{l|}{61 282} & 66 999 & \multicolumn{1}{l|}{19 133} & 24 861 & \multicolumn{1}{l|}{22 667} & 17 654 \\ \hline
Final Nb Arcs  & \multicolumn{1}{l|}{14 858}  & 121 625 & \multicolumn{1}{l|}{14 278}  & 122 068 & \multicolumn{1}{l|}{11 109}  & 57 671  & \multicolumn{1}{l|}{2 700}   & 29 828  & \multicolumn{1}{l|}{4 837}   & 22 261  & \multicolumn{1}{l|}{2 524}  & 9 129  & \multicolumn{1}{l|}{833}    & 2 566  & \multicolumn{1}{l|}{2 860}  & 1 910  \\ \hline
NC Final Arcs  & \multicolumn{1}{l|}{14 430}  & 117 679 & \multicolumn{1}{l|}{13 831}  & 119 414 & \multicolumn{1}{l|}{10 520}  & 56 856  & \multicolumn{1}{l|}{2 539}   & 29 343  & \multicolumn{1}{l|}{4 697}   & 21 894  & \multicolumn{1}{l|}{2 177}  & 8 815  & \multicolumn{1}{l|}{703}    & 2 344  & \multicolumn{1}{l|}{2 664}  & 1 576  \\ \hline
Nb Undefined   & \multicolumn{1}{l|}{144}     & 6 824   & \multicolumn{1}{l|}{328}     & 8 071   & \multicolumn{1}{l|}{89}      & 5 409   & \multicolumn{1}{l|}{46}      & 2 002   & \multicolumn{1}{l|}{22}      & 1 969   & \multicolumn{1}{l|}{48}     & 1 635  & \multicolumn{1}{l|}{33}     & 669    & \multicolumn{1}{l|}{11}     & 454    \\ \hline
Nb Undefining  & \multicolumn{1}{l|}{137 815} & 35 257  & \multicolumn{1}{l|}{86 374}  & 39 126  & \multicolumn{1}{l|}{44 280}  & 20 153  & \multicolumn{1}{l|}{33 246}  & 16 599  & \multicolumn{1}{l|}{18 843}  & 14 400  & \multicolumn{1}{l|}{9 278}  & 6 410  & \multicolumn{1}{l|}{3 261}  & 2 764  & \multicolumn{1}{l|}{1 874}  & 1 872  \\ \hline
Nb SCCs Kernel & \multicolumn{1}{l|}{253}     & 31      & \multicolumn{1}{l|}{459}     & 107     & \multicolumn{1}{l|}{385}     & 60      & \multicolumn{1}{l|}{168}     & 58      & \multicolumn{1}{l|}{65}      & 18      & \multicolumn{1}{l|}{125}    & 49     & \multicolumn{1}{l|}{49}     & 15     & \multicolumn{1}{l|}{18}     & 25     \\ \hline
\end{tabular}
\end{table}


==> latex/tables/amr_creation.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
                      & \multicolumn{2}{c|}{WordNet}           & \multicolumn{2}{c|}{MerWeb}           & \multicolumn{2}{c|}{WEDT}            & \multicolumn{2}{c|}{LDOCE}           & \multicolumn{2}{c|}{CIDE}            & \multicolumn{2}{c|}{WCDT}            & \multicolumn{2}{c|}{WLDT}          & \multicolumn{2}{c|}{WILD}          \\ \hline
Init Def. Qty         & \multicolumn{1}{l|}{todo}    & 206 185 & \multicolumn{1}{l|}{TODO}   & 301 240 & \multicolumn{1}{l|}{TODO}   & 86 949 & \multicolumn{1}{l|}{todo}   & 80 086 & \multicolumn{1}{l|}{todo}   & 49 787 & \multicolumn{1}{l|}{todo}   & 22 563 & \multicolumn{1}{l|}{todo}  & 6 900 & \multicolumn{1}{l|}{todo}  & 4 709 \\ \hline
Invalid Quantity      & \multicolumn{1}{l|}{552}     & 98 443  & \multicolumn{1}{l|}{1 127}  & 98 349  & \multicolumn{1}{l|}{907}    & 28 548 & \multicolumn{1}{l|}{394}    & 17 030 & \multicolumn{1}{l|}{187}    & 10 484 & \multicolumn{1}{l|}{466}    & 3 910  & \multicolumn{1}{l|}{213}   & 739   & \multicolumn{1}{l|}{173}   & 796   \\ \hline
Saved Quantity        & \multicolumn{1}{l|}{143 918} & 32 195  & \multicolumn{1}{l|}{94 435} & 43 632  & \multicolumn{1}{l|}{50 102} & 13 721 & \multicolumn{1}{l|}{34 782} & 9 538  & \multicolumn{1}{l|}{20 225} & 7 564  & \multicolumn{1}{l|}{11 571} & 1 936  & \multicolumn{1}{l|}{4 168} & 400   & \multicolumn{1}{l|}{2 642} & 231   \\ \hline
First Strategy        & \multicolumn{1}{l|}{5 497}   & 7 813   & \multicolumn{1}{l|}{7 523}  & 14 629  & \multicolumn{1}{l|}{5 732}  & 5 192  & \multicolumn{1}{l|}{1 727}  & 3 677  & \multicolumn{1}{l|}{1 184}  & 3 431  & \multicolumn{1}{l|}{2 827}  & 722    & \multicolumn{1}{l|}{1 085} & 182   & \multicolumn{1}{l|}{1 180} & 155   \\ \hline
Definition Strategy   & \multicolumn{1}{l|}{412}     & 24 382  & \multicolumn{1}{l|}{820}    & 29 003  & \multicolumn{1}{l|}{820}    & 8529   & \multicolumn{1}{l|}{345}    & 5 861  & \multicolumn{1}{l|}{164}    & 4 133  & \multicolumn{1}{l|}{420}    & 1 214  & \multicolumn{1}{l|}{185}   & 218   & \multicolumn{1}{l|}{161}   & 76    \\ \hline
Invalid Lost Quantity & \multicolumn{1}{l|}{4}       & 66 248  & \multicolumn{1}{l|}{2}      & 54 717  & \multicolumn{1}{l|}{5}      & 14 827 & \multicolumn{1}{l|}{3}      & 7 492  & \multicolumn{1}{l|}{2}      & 2 920  & \multicolumn{1}{l|}{7}      & 1 974  & \multicolumn{1}{l|}{1}     & 1     & \multicolumn{1}{l|}{1}     & 565   \\ \hline
Disamb Filtered       & \multicolumn{1}{l|}{457}     & 46 486  & \multicolumn{1}{l|}{940}    & 141 255 & \multicolumn{1}{l|}{441}    & 25 137 & \multicolumn{1}{l|}{205}    & 39 257 & \multicolumn{1}{l|}{118}    & 24 296 & \multicolumn{1}{l|}{394}    & 7 822  & \multicolumn{1}{l|}{206}   & 1 600 & \multicolumn{1}{l|}{133}   & 1 085 \\ \hline
Final Quantity        & \multicolumn{1}{l|}{4 093}   & 93 451  & \multicolumn{1}{l|}{5 067}  & 105 268 & \multicolumn{1}{l|}{3 789}  & 46 985 & \multicolumn{1}{l|}{966}    & 33 337 & \multicolumn{1}{l|}{723}    & 22 571 & \multicolumn{1}{l|}{1 497}  & 12 717 & \multicolumn{1}{l|}{556}   & 4 961 & \multicolumn{1}{l|}{587}   & 3 059 \\ \hline
Disamb Ratio          & \multicolumn{1}{l|}{193}     & 1.07    & \multicolumn{1}{l|}{284}    & 1.23    & \multicolumn{1}{l|}{298}    & 1.10   & \multicolumn{1}{l|}{70}     & 1.11   & \multicolumn{1}{l|}{61}     & 1.12   & \multicolumn{1}{l|}{259}    & 1.08   & \multicolumn{1}{l|}{36}    & 1.03  & \multicolumn{1}{l|}{110}   & 1.03  \\ \hline
+1 Def Qty            & \multicolumn{1}{l|}{338}     & 5 963   & \multicolumn{1}{l|}{410}    & 15 493  & \multicolumn{1}{l|}{379}    & 4 152  & \multicolumn{1}{l|}{138}    & 7 492  & \multicolumn{1}{l|}{116}    & 2 122  & \multicolumn{1}{l|}{250}    & 907    & \multicolumn{1}{l|}{96}    & 189   & \multicolumn{1}{l|}{188}   & 102   \\ \hline
\end{tabular}
\end{table}


==> latex/tables/amr_creation_results.tex <==
\begin{table}[]
	\centering
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
		\hline
		& WordNet      & MerrWeb      & WEDT        & LDOCE       & CIDE      & WCDT      & WLDT    & WILD    \\ \hline
		Definition Quantity & 146 703      & 97 715       & 52 794      & 35 834      & 21 322    & 12 579    & 4 687   & 3 366   \\ \hline
		Invalid Quantity    & 86 211       & 37 482       & 18 116      & 11 223      & 4 574     & 2 185     & 451     & 647     \\ \hline
		Saved Quantity      & 85 346       & 37 072       & 18 087      & 11 142      & 4500      & 2176      & 449     & 644     \\ \hline
		First Strategy      & 84 924 / 116 & 36 716 / 116 & 18 037 / 24 & 11 044 / 28 & 4367 / 38 & 2152 / 14 & 434 / 7 & 640 / 1 \\ \hline
		Definition Strategy & 306          & 240          & 26          & 70          & 95        & 10        & 8       & 3       \\ \hline
		Lost Quantity       & 865          & 410          & 29          & 40          & 74        & 9         & 2       & 3       \\ \hline
	\end{tabular}
\end{table}

==> latex/tables/confl_alg_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
           & \multicolumn{2}{l|}{WN}                                     & \multicolumn{2}{l|}{MW}                                    & \multicolumn{2}{l|}{LDOCE}                                 & \multicolumn{2}{l|}{CIDE}                                                       & \multicolumn{2}{l|}{WCDT}                                 & \multicolumn{2}{l|}{WEDT}                                  & \multicolumn{2}{l|}{WILD}                                & \multicolumn{2}{l|}{WLDT}                                \\ \hline
Nb incl.   & \multicolumn{1}{l|}{490}    & \cellcolor[HTML]{FFCE93}10303 & \multicolumn{1}{l|}{1068}  & \cellcolor[HTML]{FFCE93}11824 & \multicolumn{1}{l|}{339}   & \cellcolor[HTML]{FFCE93}2839  & \multicolumn{1}{l|}{171}                        & \cellcolor[HTML]{FFCE93}2647  & \multicolumn{1}{l|}{426}   & \cellcolor[HTML]{FFCE93}2271 & \multicolumn{1}{l|}{860}   & \cellcolor[HTML]{FFCE93}7669  & \multicolumn{1}{l|}{143}  & \cellcolor[HTML]{FFCE93}632  & \multicolumn{1}{l|}{205}  & \cellcolor[HTML]{FFCE93}937  \\ \hline
Nb excl.   & \multicolumn{1}{l|}{143881} & \cellcolor[HTML]{FFCE93}61486 & \multicolumn{1}{l|}{94533} & \cellcolor[HTML]{FFCE93}46676 & \multicolumn{1}{l|}{34851} & \cellcolor[HTML]{FFCE93}21513 & \multicolumn{1}{l|}{20306}                      & \cellcolor[HTML]{FFCE93}14077 & \multicolumn{1}{l|}{11622} & \cellcolor[HTML]{FFCE93}7789 & \multicolumn{1}{l|}{50146} & \cellcolor[HTML]{FFCE93}26993 & \multicolumn{1}{l|}{2618} & \cellcolor[HTML]{FFCE93}2421 & \multicolumn{1}{l|}{4243} & \cellcolor[HTML]{FFCE93}3360 \\ \hline
Nb remain. & \multicolumn{1}{l|}{2332}   & \cellcolor[HTML]{FFCE93}5063  & \multicolumn{1}{l|}{2114}  & \cellcolor[HTML]{FFCE93}4348  & \multicolumn{1}{l|}{644}   & \cellcolor[HTML]{FFCE93}1424  & \multicolumn{1}{l|}{845}                        & \cellcolor[HTML]{FFCE93}1105  & \multicolumn{1}{l|}{531}   & \cellcolor[HTML]{FFCE93}611  & \multicolumn{1}{l|}{1788}  & \cellcolor[HTML]{FFCCC9}2965  & \multicolumn{1}{l|}{605}  & \cellcolor[HTML]{FFCE93}130  & \multicolumn{1}{l|}{239}  & \cellcolor[HTML]{FFCE93}142  \\ \hline
Nb reduc.  & \multicolumn{1}{l|}{5077}   & \cellcolor[HTML]{FFCE93}3873  & \multicolumn{1}{l|}{7111}  & \cellcolor[HTML]{FFCE93}4350  & \multicolumn{1}{l|}{1495}  & \cellcolor[HTML]{FFCE93}1644  & \multicolumn{1}{l|}{1085}                       & \cellcolor[HTML]{FFCE93}1374  & \multicolumn{1}{l|}{2502}  & \cellcolor[HTML]{FFCE93}1617 & \multicolumn{1}{l|}{5444}  & \cellcolor[HTML]{FFCE93}3415  & \multicolumn{1}{l|}{906}  & \cellcolor[HTML]{FFCE93}540  & \multicolumn{1}{l|}{1000} & \cellcolor[HTML]{FFCE93}841  \\ \hline
Nb LOOP    & \multicolumn{1}{l|}{400}    & \cellcolor[HTML]{FFCE93}287   & \multicolumn{1}{l|}{820}   & \cellcolor[HTML]{FFCE93}371   & \multicolumn{1}{l|}{315}   & \cellcolor[HTML]{FFCE93}168   & \multicolumn{1}{l|}{158}                        & \cellcolor[HTML]{FFCE93}101   & \multicolumn{1}{l|}{419}   & \cellcolor[HTML]{FFCE93}244  & \multicolumn{1}{l|}{815}   & \cellcolor[HTML]{FFCE93}370   & \multicolumn{1}{l|}{142}  & \cellcolor[HTML]{FFCE93}75   & \multicolumn{1}{l|}{200}  & \cellcolor[HTML]{FFCE93}144  \\ \hline
Nb SUBSET  & \multicolumn{1}{l|}{2}      & \cellcolor[HTML]{FFCE93}3     & \multicolumn{1}{l|}{2}     & \cellcolor[HTML]{FFCE93}0     & \multicolumn{1}{l|}{1}     & \cellcolor[HTML]{FFCE93}0     & \multicolumn{1}{l|}{2}                          & \cellcolor[HTML]{FFCE93}0     & \multicolumn{1}{l|}{3}     & \cellcolor[HTML]{FFCE93}0    & \multicolumn{1}{l|}{4}     & \cellcolor[HTML]{FFCE93}2     & \multicolumn{1}{l|}{1}    & \cellcolor[HTML]{FFCE93}0    & \multicolumn{1}{l|}{3}    & \cellcolor[HTML]{FFCE93}0    \\ \hline
Nb IN      & \multicolumn{1}{l|}{255}    & \cellcolor[HTML]{FFCE93}317   & \multicolumn{1}{l|}{799}   & \cellcolor[HTML]{FFCE93}600   & \multicolumn{1}{l|}{114}   & \cellcolor[HTML]{FFCE93}87    & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}60} & \cellcolor[HTML]{FFCE93}79    & \multicolumn{1}{l|}{229}   & \cellcolor[HTML]{FFCE93}206  & \multicolumn{1}{l|}{281}   & \cellcolor[HTML]{FFCE93}411   & \multicolumn{1}{l|}{52}   & \cellcolor[HTML]{FFCE93}76   & \multicolumn{1}{l|}{123}  & \cellcolor[HTML]{FFCE93}139  \\ \hline
Nb OUT     & \multicolumn{1}{l|}{4195}   & \cellcolor[HTML]{FFCE93}3182  & \multicolumn{1}{l|}{5192}  & \cellcolor[HTML]{FFCE93}3279  & \multicolumn{1}{l|}{992}   & \cellcolor[HTML]{FFCE93}1344  & \multicolumn{1}{l|}{752}                        & \cellcolor[HTML]{FFCE93}755   & \multicolumn{1}{l|}{1622}  & \cellcolor[HTML]{FFCE93}1143 & \multicolumn{1}{l|}{3880}  & \cellcolor[HTML]{FFCE93}2460  & \multicolumn{1}{l|}{591}  & \cellcolor[HTML]{FFCE93}374  & \multicolumn{1}{l|}{644}  & \cellcolor[HTML]{FFCE93}545  \\ \hline
Nb PIE     & \multicolumn{1}{l|}{225}    & \cellcolor[HTML]{FFCE93}84    & \multicolumn{1}{l|}{298}   & \cellcolor[HTML]{FFCE93}100   & \multicolumn{1}{l|}{73}    & \cellcolor[HTML]{FFCE93}45    & \multicolumn{1}{l|}{113}                        & \cellcolor[HTML]{FFCE93}439   & \multicolumn{1}{l|}{229}   & \cellcolor[HTML]{FFCE93}24   & \multicolumn{1}{l|}{464}   & \cellcolor[HTML]{FFCE93}172   & \multicolumn{1}{l|}{120}  & \cellcolor[HTML]{FFCE93}15   & \multicolumn{1}{l|}{30}   & \cellcolor[HTML]{FFCE93}13   \\ \hline
\end{tabular}
\end{table}

==> latex/tables/dico-dicoAMR-conf-alg-res.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
           & \multicolumn{2}{l|}{WordNet}          & \multicolumn{2}{l|}{MerWeb}          & \multicolumn{2}{l|}{WEDT}            & \multicolumn{2}{l|}{LDOCE}           & \multicolumn{2}{l|}{CIDE}            & \multicolumn{2}{l|}{WCDT}           & \multicolumn{2}{l|}{WLDT}          & \multicolumn{2}{l|}{WILD}          \\ \hline
Nb Remain. & \multicolumn{1}{l|}{2 068}   & 5 022  & \multicolumn{1}{l|}{1 968}  & 4 308  & \multicolumn{1}{l|}{1 601}  & 2 946  & \multicolumn{1}{l|}{436}    & 1 373  & \multicolumn{1}{l|}{696}    & 1 098  & \multicolumn{1}{l|}{389}    & 598   & \multicolumn{1}{l|}{151}   & 115   & \multicolumn{1}{l|}{408}   & 130   \\ \hline
Nb Incl.   & \multicolumn{1}{l|}{548}     &        & \multicolumn{1}{l|}{1 125}  & 11 830 & \multicolumn{1}{l|}{899}    & 7 672  & \multicolumn{1}{l|}{390}    & 2 848  & \multicolumn{1}{l|}{185}    & 2 647  & \multicolumn{1}{l|}{460}    & 2 274 & \multicolumn{1}{l|}{208}   & 943   & \multicolumn{1}{l|}{172}   & 632   \\ \hline
Nb Excl.   & \multicolumn{1}{l|}{143 882} & 61 523 & \multicolumn{1}{l|}{94 402} & 46 710 & \multicolumn{1}{l|}{50 065} & 27 009 & \multicolumn{1}{l|}{34 773} & 21 538 & \multicolumn{1}{l|}{20 214} & 14 084 & \multicolumn{1}{l|}{11 530} & 7 799 & \multicolumn{1}{l|}{4 149} & 3 381 & \multicolumn{1}{l|}{2 633} & 2 421 \\ \hline
Nb Reduc   & \multicolumn{1}{l|}{5 120}   & 4 732  & \multicolumn{1}{l|}{7 079}  & 5 069  & \multicolumn{1}{l|}{5 289}  & 3 884  & \multicolumn{1}{l|}{1 576}  & 1 997  & \multicolumn{1}{l|}{1 055}  & 1 620  & \multicolumn{1}{l|}{2 531}  & 1 772 & \multicolumn{1}{l|}{965}   & 997   & \multicolumn{1}{l|}{982}   & 606   \\ \hline
Nb LOOP    & \multicolumn{1}{l|}{409}     & 290    & \multicolumn{1}{l|}{818}    & 376    & \multicolumn{1}{l|}{814}    & 373    & \multicolumn{1}{l|}{341}    & 172    & \multicolumn{1}{l|}{162}    & 101    & \multicolumn{1}{l|}{415}    & 247   & \multicolumn{1}{l|}{185}   & 148   & \multicolumn{1}{l|}{160}   & 75    \\ \hline
Nb SUBSET  & \multicolumn{1}{l|}{3}       & 4      & \multicolumn{1}{l|}{2}      & 1      & \multicolumn{1}{l|}{3}      & 2      & \multicolumn{1}{l|}{3}      & 0      & \multicolumn{1}{l|}{2}      & 0      & \multicolumn{1}{l|}{4}      & 0     & \multicolumn{1}{l|}{1}     & 2     & \multicolumn{1}{l|}{1}     & 0     \\ \hline
Nb IN      & \multicolumn{1}{l|}{431}     & 335    & \multicolumn{1}{l|}{924}    & 621    & \multicolumn{1}{l|}{427}    & 420    & \multicolumn{1}{l|}{199}    & 96     & \multicolumn{1}{l|}{113}    & 83     & \multicolumn{1}{l|}{374}    & 213   & \multicolumn{1}{l|}{193}   & 153   & \multicolumn{1}{l|}{126}   & 76    \\ \hline
Nb OUT     & \multicolumn{1}{l|}{4 084}   & 3 200  & \multicolumn{1}{l|}{5 051}  & 3 291  & \multicolumn{1}{l|}{3 763}  & 2 467  & \multicolumn{1}{l|}{963}    & 1 373  & \multicolumn{1}{l|}{717}    & 758    & \multicolumn{1}{l|}{1 477}  & 1 146 & \multicolumn{1}{l|}{550}   & 549   & \multicolumn{1}{l|}{585}   & 374   \\ \hline
Nb PIE     & \multicolumn{1}{l|}{193}     & 84     & \multicolumn{1}{l|}{284}    & 100    & \multicolumn{1}{l|}{282}    & 172    & \multicolumn{1}{l|}{70}     & 25     & \multicolumn{1}{l|}{61}     & 439    & \multicolumn{1}{l|}{259}    & 24    & \multicolumn{1}{l|}{36}    & 13    & \multicolumn{1}{l|}{110}   & 15    \\ \hline
\end{tabular}
\end{table}


==> latex/tables/dico-dicoAMR_graph_metrics.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
               & \multicolumn{2}{l|}{WordNet}           & \multicolumn{2}{l|}{MerWeb}            & \multicolumn{2}{l|}{WEDT}              & \multicolumn{2}{l|}{CIDE}              & \multicolumn{2}{l|}{LDOCE}             & \multicolumn{2}{l|}{WILD}            & \multicolumn{2}{l|}{WCDT}            & \multicolumn{2}{l|}{WLDT}            \\ \hline
Nb vertices    & \multicolumn{1}{l|}{146 498} & 76 852  & \multicolumn{1}{l|}{97 945}  & 62 848  & \multicolumn{1}{l|}{52 565}  & 37 627  & \multicolumn{1}{l|}{21 095}  & 25 759  & \multicolumn{1}{l|}{35 599}  & 17 829  & \multicolumn{1}{l|}{3 213}  & 10 671 & \multicolumn{1}{l|}{12 379} & 4 439  & \multicolumn{1}{l|}{4 508}  & 3 183  \\ \hline
Size Kernel    & \multicolumn{1}{l|}{7 131}   & 18 865  & \multicolumn{1}{l|}{9 070}   & 20 051  & \multicolumn{1}{l|}{6 694}   & 13 505  & \multicolumn{1}{l|}{1 711}   & 5 690   & \multicolumn{1}{l|}{1 988}   & 4 586   & \multicolumn{1}{l|}{1 291}  & 4 231  & \multicolumn{1}{l|}{2 183}  & 1 763  & \multicolumn{1}{l|}{1 103}  & 1212   \\ \hline
Size Red. Ker. & \multicolumn{1}{l|}{2 068}   & 5 063   & \multicolumn{1}{l|}{1 968}   & 4 348   & \multicolumn{1}{l|}{1 601}   & 2965    & \multicolumn{1}{l|}{696}     & 1 377   & \multicolumn{1}{l|}{436}     & 1105    & \multicolumn{1}{l|}{408}    & 611    & \multicolumn{1}{l|}{389}    & 142    & \multicolumn{1}{l|}{147}    & 130    \\ \hline
NC Red Ker.    & \multicolumn{1}{l|}{2 028}   & todo    & \multicolumn{1}{l|}{1 933}   & todo    & \multicolumn{1}{l|}{1 556}   & todo    & \multicolumn{1}{l|}{683}     &         & \multicolumn{1}{l|}{423}     & todo    & \multicolumn{1}{l|}{398}    & todo   & \multicolumn{1}{l|}{342}    & todo   & \multicolumn{1}{l|}{123}    & todo   \\ \hline
Init. Nb Arcs  & \multicolumn{1}{l|}{765 481} & 606 727 & \multicolumn{1}{l|}{495 385} & 458 314 & \multicolumn{1}{l|}{273 432} & 271 776 & \multicolumn{1}{l|}{107 638} & 211 738 & \multicolumn{1}{l|}{173 737} & 149 731 & \multicolumn{1}{l|}{22 667} & 63 961 & \multicolumn{1}{l|}{61 282} & 23 419 & \multicolumn{1}{l|}{19 133} & 17 211 \\ \hline
Final Nb Arcs  & \multicolumn{1}{l|}{14 858}  & 87 701  & \multicolumn{1}{l|}{14 278}  & 71 462  & \multicolumn{1}{l|}{11 109}  & 403 395 & \multicolumn{1}{l|}{4 837}   & 20 950  & \multicolumn{1}{l|}{2 700}   & 14 531  & \multicolumn{1}{l|}{2 860}  & 6 278  & \multicolumn{1}{l|}{2 524}  & 1 684  & \multicolumn{1}{l|}{833}    & 1 286  \\ \hline
NC Final Arcs  & \multicolumn{1}{l|}{14 430}  & todo    & \multicolumn{1}{l|}{13 831}  & todo    & \multicolumn{1}{l|}{10 520}  & todo    & \multicolumn{1}{l|}{4 697}   & todo    & \multicolumn{1}{l|}{2 539}   & todo    & \multicolumn{1}{l|}{2 664}  & todo   & \multicolumn{1}{l|}{2 177}  & todo   & \multicolumn{1}{l|}{703}    & todo   \\ \hline
Nb Undefined   & \multicolumn{1}{l|}{144}     & 10 067  & \multicolumn{1}{l|}{328}     & 11 644  & \multicolumn{1}{l|}{89}      & 7 381   & \multicolumn{1}{l|}{22}      & 2 701   & \multicolumn{1}{l|}{46}      & 2 558   & \multicolumn{1}{l|}{11}     & 2 056  & \multicolumn{1}{l|}{48}     & 809    & \multicolumn{1}{l|}{33}     & 568    \\ \hline
Nb Undefining  & \multicolumn{1}{l|}{137 815} & 57 672  & \multicolumn{1}{l|}{86 374}  & 41 603  & \multicolumn{1}{l|}{44 280}  & 23 696  & \multicolumn{1}{l|}{18 843}  & 19 931  & \multicolumn{1}{l|}{33 246}  & 13 012  & \multicolumn{1}{l|}{1 874}  & 6 347  & \multicolumn{1}{l|}{9 278}  & 2 643  & \multicolumn{1}{l|}{3 261}  & 1 946  \\ \hline
Nb SCCs Kernel & \multicolumn{1}{l|}{253}     & 26      & \multicolumn{1}{l|}{459}     & 58      & \multicolumn{1}{l|}{385}     & 43      & \multicolumn{1}{l|}{65}      & 44      & \multicolumn{1}{l|}{168}     & 19      & \multicolumn{1}{l|}{18}     & 44     & \multicolumn{1}{l|}{125}    & 13     & \multicolumn{1}{l|}{49}     & 15     \\ \hline
\end{tabular}
\end{table}


==> latex/tables/dicoAMR_disamb_graph_metrics.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
                 & WordNet & MerrWeb & WEDT    & LDOCE   & CIDE    & WCDT   & WLDT   & WILD   \\ \hline
Nb Vertices      & 45 488  & 55 649  & 31 258  & 20 602  & 17 709  & 10 407 & 4 485  & 3 184  \\ \hline
Nb Kernel        & 21 644  & 24 093  & 15 578  & 5 892   & 5 154   & 4 668  & 1 777  & 1 302  \\ \hline
Size Red. Kernel & 7 800   & 7 586   & 4 833   & 2031    & 1 719   & 1 222  & 300    & 299    \\ \hline
NC Red. Kernel   & 7 725   & 7 496   & 4 785   & 2 021   & 1 711   & 1 191  & 283    & 225    \\ \hline
Init Nb Arcs     & 478 133 & 479 228 & 263 966 & 202 711 & 164 304 & 68 043 & 23 234 & 18 196 \\ \hline
Final Nb Arcs    & 178 727 & 158 599 & 82 423  & 42 883  & 28 689  & 12 497 & 2 718  & 2 545  \\ \hline
NC Final Arcs    & 175 725 & 155 268 & 80 898  & 41 624  & 27 787  & 11 934 & 2 523  & 1 866  \\ \hline
Nb Undefined     & 7 611   & 9 291   & 5 950   & 1 838   & 1 894   & 1 545  & 632    & 480    \\ \hline
Nb Undefining    & 23 213  & 29 841  & 15 092  & 14 509  & 12 319  & 5 654  & 2 683  & 1 846  \\ \hline
Nb SCCs Kernel   & 6       & 43      & 32      & 49      & 18      & 31     & 19     & 14     \\ \hline
\end{tabular}
\end{table}


==> latex/tables/graph_metrics.tex <==
\begin{table}[]
	\centering
	\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
		\hline
		& \multicolumn{2}{l|}{WordNet}           & \multicolumn{2}{l|}{MerWeb}            & \multicolumn{2}{l|}{WEDT}              & \multicolumn{2}{l|}{LDOCE}             & \multicolumn{2}{l|}{CIDE}              & \multicolumn{2}{l|}{WCDT}            & \multicolumn{2}{l|}{WLDT}            & \multicolumn{2}{l|}{WILD}            \\ \hline
		Nb vertices    & \multicolumn{1}{l|}{146 703} & 76 852  & \multicolumn{1}{l|}{97 715}  & 62 848  & \multicolumn{1}{l|}{52 794}  & 37 627  & \multicolumn{1}{l|}{21322}   & 25 759  & \multicolumn{1}{l|}{35 834}  & 17 829  & \multicolumn{1}{l|}{3 366}  & 10 671 & \multicolumn{1}{l|}{12 579} & 4 439  & \multicolumn{1}{l|}{4 687}  & 3 183  \\ \hline
		Size Kernel    & \multicolumn{1}{l|}{7 272}   & 18 865  & \multicolumn{1}{l|}{9 173}   & 20 051  & \multicolumn{1}{l|}{6 809}   & 13 505  & \multicolumn{1}{l|}{1 828}   & 5 690   & \multicolumn{1}{l|}{2 089}   & 4 586   & \multicolumn{1}{l|}{1 391}  & 4 231  & \multicolumn{1}{l|}{2 808}  & 1 763  & \multicolumn{1}{l|}{1 211}  & 1212   \\ \hline
		Size Core      & \multicolumn{1}{l|}{5 466}   & 8 791   & \multicolumn{1}{l|}{6 522}   & 8 406   & \multicolumn{1}{l|}{5 119}   & 6 059   & \multicolumn{1}{l|}{1 617}   & 2 895   & \multicolumn{1}{l|}{1 577}   & 1 972   & \multicolumn{1}{l|}{1 332}  & 2 062  & \multicolumn{1}{l|}{2 331}  & 916    & \multicolumn{1}{l|}{1 025}  & 619    \\ \hline
		Size Red. Core & \multicolumn{1}{l|}{2 332}   & 5 063   & \multicolumn{1}{l|}{2 114}   & 4 348   & \multicolumn{1}{l|}{1 788}   & 2965    & \multicolumn{1}{l|}{845}     & 1 377   & \multicolumn{1}{l|}{644}     & 1105    & \multicolumn{1}{l|}{605}    & 611    & \multicolumn{1}{l|}{531}    & 142    & \multicolumn{1}{l|}{239}    & 130    \\ \hline
		Nb. Nodes Sat. & \multicolumn{1}{l|}{572}     & 53      & \multicolumn{1}{l|}{1054}    & 144     & \multicolumn{1}{l|}{858}     & 119     & \multicolumn{1}{l|}{139}     & 99      & \multicolumn{1}{l|}{339}     & 48      & \multicolumn{1}{l|}{30}     & 115    & \multicolumn{1}{l|}{269}    & 42     & \multicolumn{1}{l|}{109}    & 25     \\ \hline
		Init. Nb Arcs  & \multicolumn{1}{l|}{818 569} & 606 727 & \multicolumn{1}{l|}{533 686} & 458 314 & \multicolumn{1}{l|}{297 930} & 271 776 & \multicolumn{1}{l|}{127 401} & 211 738 & \multicolumn{1}{l|}{199 612} & 149 731 & \multicolumn{1}{l|}{30 454} & 63 961 & \multicolumn{1}{l|}{71 436} & 23 419 & \multicolumn{1}{l|}{23 254} & 17 211 \\ \hline
		Final Nb Arcs  & \multicolumn{1}{l|}{17 736}  & 87 701  & \multicolumn{1}{l|}{15 806}  & 71 462  & \multicolumn{1}{l|}{13 372}  & 403 395 & \multicolumn{1}{l|}{6 874}   & 20 950  & \multicolumn{1}{l|}{4 381}   & 14 531  & \multicolumn{1}{l|}{5 409}  & 6 278  & \multicolumn{1}{l|}{3 592}  & 1 684  & \multicolumn{1}{l|}{1 434}  & 1 286  \\ \hline
		Nb Undefined   & \multicolumn{1}{l|}{89}      & 10 067  & \multicolumn{1}{l|}{264}     & 11 644  & \multicolumn{1}{l|}{42}      & 7 381   & \multicolumn{1}{l|}{12}      & 2 701   & \multicolumn{1}{l|}{23}      & 2 558   & \multicolumn{1}{l|}{0}      & 2 056  & \multicolumn{1}{l|}{5}      & 809    & \multicolumn{1}{l|}{2}      & 568    \\ \hline
		Nb Undefining  & \multicolumn{1}{l|}{138 296} & 57 672  & \multicolumn{1}{l|}{86 754}  & 41 603  & \multicolumn{1}{l|}{44 612}  & 23 696  & \multicolumn{1}{l|}{19 114}  & 19 931  & \multicolumn{1}{l|}{33 495}  & 13 012  & \multicolumn{1}{l|}{1 929}  & 6 347  & \multicolumn{1}{l|}{9 4 14} & 2 643  & \multicolumn{1}{l|}{3 365}  & 1 946  \\ \hline
		Nb SCCs Kernel & \multicolumn{1}{l|}{249}     & 27      & \multicolumn{1}{l|}{458}     & 70      & \multicolumn{1}{l|}{388}     & 57      & \multicolumn{1}{l|}{64}      & 50      & \multicolumn{1}{l|}{167}     & 23      & \multicolumn{1}{l|}{15}     & 52     & \multicolumn{1}{l|}{121}    & 19     & \multicolumn{1}{l|}{48}     & 13     \\ \hline
	\end{tabular}
\end{table}

==> latex/tables/nc_3_types_graph.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|lll|lll|lll|lll|lll|lll|lll|lll|}
\hline
           & \multicolumn{3}{c|}{WordNet}                                      & \multicolumn{3}{c|}{MerWeb}                                      & \multicolumn{3}{c|}{WEDT}                                          & \multicolumn{3}{c|}{LDOCE}                                         & \multicolumn{3}{c|}{CIDE}                                          & \multicolumn{3}{c|}{WCDT}                                        & \multicolumn{3}{c|}{WLDT}                                       & \multicolumn{3}{c|}{WILD}                                       \\ \hline
Nb Remain. & \multicolumn{1}{l|}{2 028}   & \multicolumn{1}{l|}{TODO} & 6 428  & \multicolumn{1}{l|}{1 933}  & \multicolumn{1}{l|}{TODO} & 6 607  & \multicolumn{1}{l|}{1 556}  & \multicolumn{1}{l|}{4 785}  & 3 858  & \multicolumn{1}{l|}{423}    & \multicolumn{1}{l|}{2 021}  & 1 738  & \multicolumn{1}{l|}{683}    & \multicolumn{1}{l|}{1 711}  & 1 482  & \multicolumn{1}{l|}{342}    & \multicolumn{1}{l|}{1 191} & 935   & \multicolumn{1}{l|}{127}   & \multicolumn{1}{l|}{283}   & 272   & \multicolumn{1}{l|}{398}   & \multicolumn{1}{l|}{0}     & 192   \\ \hline
Nb Incl.   & \multicolumn{1}{l|}{552}     & \multicolumn{1}{l|}{}     & 7 257  & \multicolumn{1}{l|}{1 127}  & \multicolumn{1}{l|}{}     & 8 637  & \multicolumn{1}{l|}{907}    & \multicolumn{1}{l|}{6 389}  & 5 878  & \multicolumn{1}{l|}{394}    & \multicolumn{1}{l|}{2 075}  & 2 226  & \multicolumn{1}{l|}{187}    & \multicolumn{1}{l|}{2 030}  & 2 102  & \multicolumn{1}{l|}{466}    & \multicolumn{1}{l|}{1 807} & 1 909 & \multicolumn{1}{l|}{213}   & \multicolumn{1}{l|}{782}   & 810   & \multicolumn{1}{l|}{173}   & \multicolumn{1}{l|}{678}   & 540   \\ \hline
Nb Excl.   & \multicolumn{1}{l|}{143 918} & \multicolumn{1}{l|}{}     & 40 896 & \multicolumn{1}{l|}{94 435} & \multicolumn{1}{l|}{}     & 46 619 & \multicolumn{1}{l|}{50 102} & \multicolumn{1}{l|}{20 084} & 24 247 & \multicolumn{1}{l|}{34 782} & \multicolumn{1}{l|}{16 506} & 18 688 & \multicolumn{1}{l|}{20 225} & \multicolumn{1}{l|}{13 968} & 15 791 & \multicolumn{1}{l|}{11 571} & \multicolumn{1}{l|}{7 409} & 8 085 & \multicolumn{1}{l|}{4 168} & \multicolumn{1}{l|}{3 420} & 3 500 & \multicolumn{1}{l|}{2 642} & \multicolumn{1}{l|}{2 305} & 2 399 \\ \hline
Nb Reduc   & \multicolumn{1}{l|}{5 497}   & \multicolumn{1}{l|}{}     & 8 495  & \multicolumn{1}{l|}{7 523}  & \multicolumn{1}{l|}{}     & 8 916  & \multicolumn{1}{l|}{5 732}  & \multicolumn{1}{l|}{6 438}  & 5 422  & \multicolumn{1}{l|}{1 727}  & \multicolumn{1}{l|}{2 021}  & 2 760  & \multicolumn{1}{l|}{1 184}  & \multicolumn{1}{l|}{2 669}  & 1 800  & \multicolumn{1}{l|}{2 827}  & \multicolumn{1}{l|}{2 397} & 2 304 & \multicolumn{1}{l|}{1 085} & \multicolumn{1}{l|}{1 046} & 1 093 & \multicolumn{1}{l|}{1 180} & \multicolumn{1}{l|}{587}   & 1 019 \\ \hline
Nb LOOP    & \multicolumn{1}{l|}{412}     & \multicolumn{1}{l|}{}     & 455    & \multicolumn{1}{l|}{820}    & \multicolumn{1}{l|}{}     & 639    & \multicolumn{1}{l|}{820}    & \multicolumn{1}{l|}{466}    & 503    & \multicolumn{1}{l|}{345}    & \multicolumn{1}{l|}{240}    & 228    & \multicolumn{1}{l|}{164}    & \multicolumn{1}{l|}{130}    & 135    & \multicolumn{1}{l|}{420}    & \multicolumn{1}{l|}{261}   & 281   & \multicolumn{1}{l|}{185}   & \multicolumn{1}{l|}{154}   & 149   & \multicolumn{1}{l|}{161}   & \multicolumn{1}{l|}{96}    & 85    \\ \hline
Nb SUBSET  & \multicolumn{1}{l|}{4}       & \multicolumn{1}{l|}{}     & 5      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{}     & 4      & \multicolumn{1}{l|}{5}      & \multicolumn{1}{l|}{5}      & 3      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & 1      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{0}      & 0      & \multicolumn{1}{l|}{7}      & \multicolumn{1}{l|}{5}     & 1     & \multicolumn{1}{l|}{1}     & \multicolumn{1}{l|}{1}     & 1     & \multicolumn{1}{l|}{1}     & \multicolumn{1}{l|}{0}     & 1     \\ \hline
Nb IN      & \multicolumn{1}{l|}{457}     & \multicolumn{1}{l|}{}     & 383    & \multicolumn{1}{l|}{940}    & \multicolumn{1}{l|}{}     & 888    & \multicolumn{1}{l|}{441}    & \multicolumn{1}{l|}{308}    & 313    & \multicolumn{1}{l|}{205}    & \multicolumn{1}{l|}{67}     & 85     & \multicolumn{1}{l|}{118}    & \multicolumn{1}{l|}{55}     & 65     & \multicolumn{1}{l|}{394}    & \multicolumn{1}{l|}{170}   & 185   & \multicolumn{1}{l|}{206}   & \multicolumn{1}{l|}{105}   & 111   & \multicolumn{1}{l|}{133}   & \multicolumn{1}{l|}{160}   & 78    \\ \hline
Nb OUT     & \multicolumn{1}{l|}{4 093}   & \multicolumn{1}{l|}{}     & 5 010  & \multicolumn{1}{l|}{5 067}  & \multicolumn{1}{l|}{}     & 5 711  & \multicolumn{1}{l|}{3 789}  & \multicolumn{1}{l|}{4 093}  & 3 568  & \multicolumn{1}{l|}{966}    & \multicolumn{1}{l|}{1 720}  & 1 915  & \multicolumn{1}{l|}{723}    & \multicolumn{1}{l|}{1 358}  & 1 205  & \multicolumn{1}{l|}{1 497}  & \multicolumn{1}{l|}{1 500} & 1 466 & \multicolumn{1}{l|}{556}   & \multicolumn{1}{l|}{605}   & 607   & \multicolumn{1}{l|}{587}   & \multicolumn{1}{l|}{331}   & 442   \\ \hline
Nb PIE     & \multicolumn{1}{l|}{193}     & \multicolumn{1}{l|}{}     & 1 163  & \multicolumn{1}{l|}{284}    & \multicolumn{1}{l|}{}     & 364    & \multicolumn{1}{l|}{298}    & \multicolumn{1}{l|}{345}    & 312    & \multicolumn{1}{l|}{70}     & \multicolumn{1}{l|}{94}     & 52     & \multicolumn{1}{l|}{61}     & \multicolumn{1}{l|}{232}    & 32     & \multicolumn{1}{l|}{259}    & \multicolumn{1}{l|}{58}    & 86    & \multicolumn{1}{l|}{36}    & \multicolumn{1}{l|}{5}     & 60    & \multicolumn{1}{l|}{110}   & \multicolumn{1}{l|}{0}     & 177   \\ \hline
Nb DOME++  & \multicolumn{1}{l|}{338}     & \multicolumn{1}{l|}{}     & 1 479  & \multicolumn{1}{l|}{410}    & \multicolumn{1}{l|}{}     & 1 310  & \multicolumn{1}{l|}{379}    & \multicolumn{1}{l|}{1 221}  & 723    & \multicolumn{1}{l|}{138}    & \multicolumn{1}{l|}{1 230}  & 479    & \multicolumn{1}{l|}{116}    & \multicolumn{1}{l|}{894}    & 363    & \multicolumn{1}{l|}{250}    & \multicolumn{1}{l|}{403}   & 285   & \multicolumn{1}{l|}{96}    & \multicolumn{1}{l|}{175}   & 165   & \multicolumn{1}{l|}{188}   & \multicolumn{1}{l|}{0}     & 236   \\ \hline
\end{tabular}
\end{table}


==> latex/tables/nc_two_graphs_metrics.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
           & \multicolumn{2}{c|}{WordNet}          & \multicolumn{2}{c|}{MerWeb}          & \multicolumn{2}{c|}{WEDT}            & \multicolumn{2}{c|}{LDOCE}           & \multicolumn{2}{c|}{CIDE}            & \multicolumn{2}{c|}{WCDT}           & \multicolumn{2}{c|}{WLDT}          & \multicolumn{2}{c|}{WILD}          \\ \hline
Nb Remain. & \multicolumn{1}{l|}{2 028}   & 2 928  & \multicolumn{1}{l|}{1 933}  & 2 807  & \multicolumn{1}{l|}{1 556}  & 1 822  & \multicolumn{1}{l|}{423}    & 915    & \multicolumn{1}{l|}{683}    & 1 058  & \multicolumn{1}{l|}{342}    & 353   & \multicolumn{1}{l|}{127}   & 85    & \multicolumn{1}{l|}{398}   & 184   \\ \hline
Nb Incl.   & \multicolumn{1}{l|}{552}     & 4 697  & \multicolumn{1}{l|}{1 127}  & 6 234  & \multicolumn{1}{l|}{907}    & 4 466  & \multicolumn{1}{l|}{394}    & 1 412  & \multicolumn{1}{l|}{187}    & 1 644  & \multicolumn{1}{l|}{466}    & 1 594 & \multicolumn{1}{l|}{213}   & 693   & \multicolumn{1}{l|}{173}   & 466   \\ \hline
Nb Excl.   & \multicolumn{1}{l|}{143 918} & 44 528 & \multicolumn{1}{l|}{94 435} & 50 370 & \multicolumn{1}{l|}{50 102} & 26 362 & \multicolumn{1}{l|}{34 782} & 19 542 & \multicolumn{1}{l|}{20 225} & 16 210 & \multicolumn{1}{l|}{11 571} & 8 673 & \multicolumn{1}{l|}{4 168} & 3 697 & \multicolumn{1}{l|}{2 642} & 2 414 \\ \hline
Nb Reduc   & \multicolumn{1}{l|}{5 498}   & 4 481  & \multicolumn{1}{l|}{7 526}  & 5 421  & \multicolumn{1}{l|}{5 733}  & 3 653  & \multicolumn{1}{l|}{1 727}  & 1 488  & \multicolumn{1}{l|}{1 184}  & 1 253  & \multicolumn{1}{l|}{2 828}  & 1 721 & \multicolumn{1}{l|}{1 086} & 879   & \multicolumn{1}{l|}{1 180} & 827   \\ \hline
Nb LOOP    & \multicolumn{1}{l|}{412}     & 258    & \multicolumn{1}{l|}{820}    & 418    & \multicolumn{1}{l|}{820}    & 361    & \multicolumn{1}{l|}{345}    & 156    & \multicolumn{1}{l|}{164}    & 93     & \multicolumn{1}{l|}{420}    & 256   & \multicolumn{1}{l|}{185}   & 134   & \multicolumn{1}{l|}{161}   & 77    \\ \hline
Nb SUBSET  & \multicolumn{1}{l|}{4}       & 1      & \multicolumn{1}{l|}{2}      & 0      & \multicolumn{1}{l|}{5}      & 0      & \multicolumn{1}{l|}{3}      & 0      & \multicolumn{1}{l|}{2}      & 1      & \multicolumn{1}{l|}{7}      & 2     & \multicolumn{1}{l|}{1}     & 1     & \multicolumn{1}{l|}{1}     & 0     \\ \hline
Nb IN      & \multicolumn{1}{l|}{457}     & 504    & \multicolumn{1}{l|}{940}    & 945    & \multicolumn{1}{l|}{441}    & 442    & \multicolumn{1}{l|}{205}    & 155    & \multicolumn{1}{l|}{118}    & 117    & \multicolumn{1}{l|}{394}    & 185   & \multicolumn{1}{l|}{206}   & 111   & \multicolumn{1}{l|}{133}   & 53    \\ \hline
Nb OUT     & \multicolumn{1}{l|}{4 093}   & 3 146  & \multicolumn{1}{l|}{5 067}  & 3 509  & \multicolumn{1}{l|}{3 789}  & 2 418  & \multicolumn{1}{l|}{966}    & 968    & \multicolumn{1}{l|}{723}    & 783    & \multicolumn{1}{l|}{1 497}  & 1 085 & \multicolumn{1}{l|}{556}   & 607   & \multicolumn{1}{l|}{587}   & 364   \\ \hline
Nb PIE     & \multicolumn{1}{l|}{193}     & 78     & \multicolumn{1}{l|}{284}    & 46     & \multicolumn{1}{l|}{298}    & 179    & \multicolumn{1}{l|}{70}     & 28     & \multicolumn{1}{l|}{61}     & 13     & \multicolumn{1}{l|}{259}    & 3     & \multicolumn{1}{l|}{36}    & 60    & \multicolumn{1}{l|}{110}   & 4     \\ \hline
Nb DOME++  & \multicolumn{1}{l|}{338}     & 492    & \multicolumn{1}{l|}{410}    & 503    & \multicolumn{1}{l|}{379}    & 253    & \multicolumn{1}{l|}{138}    & 181    & \multicolumn{1}{l|}{116}    & 246    & \multicolumn{1}{l|}{250}    & 155   & \multicolumn{1}{l|}{96}    & 165   & \multicolumn{1}{l|}{188}   & 328   \\ \hline
Nb ISOL.   & \multicolumn{1}{l|}{1}       & 2      & \multicolumn{1}{l|}{3}      & 0      & \multicolumn{1}{l|}{1}      & 0      & \multicolumn{1}{l|}{0}      & 0      & \multicolumn{1}{l|}{0}      & 0      & \multicolumn{1}{l|}{1}      & 0     & \multicolumn{1}{l|}{1}     & 0     & \multicolumn{1}{l|}{0}     & 1     \\ \hline
\end{tabular}
\end{table}


==> latex/tables/two_graph_confl.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
           & \multicolumn{2}{c|}{WordNet}          & \multicolumn{2}{c|}{MerWeb}          & \multicolumn{2}{c|}{WEDT}            & \multicolumn{2}{c|}{LDOCE}           & \multicolumn{2}{c|}{CIDE}            & \multicolumn{2}{c|}{WCDT}           & \multicolumn{2}{c|}{WLDT}          & \multicolumn{2}{c|}{WILD}          \\ \hline
Nb Remain. & \multicolumn{1}{l|}{2 068}   & 2 948  & \multicolumn{1}{l|}{1 968}  & 2 846  & \multicolumn{1}{l|}{1 601}  & 1 836  & \multicolumn{1}{l|}{436}    & 931    & \multicolumn{1}{l|}{696}    & 1 067  & \multicolumn{1}{l|}{389}    & 374   & \multicolumn{1}{l|}{151}   & 95    & \multicolumn{1}{l|}{408}   & 216   \\ \hline
Nb Incl.   & \multicolumn{1}{l|}{548}     & 4 697  & \multicolumn{1}{l|}{1 125}  & 6 233  & \multicolumn{1}{l|}{899}    & 4 465  & \multicolumn{1}{l|}{390}    & 1 411  & \multicolumn{1}{l|}{185}    & 1 643  & \multicolumn{1}{l|}{460}    & 1 591 & \multicolumn{1}{l|}{208}   & 692   & \multicolumn{1}{l|}{172}   & 457   \\ \hline
Nb Excl.   & \multicolumn{1}{l|}{143 882} & 44 508 & \multicolumn{1}{l|}{94 402} & 50 332 & \multicolumn{1}{l|}{50 065} & 26 349 & \multicolumn{1}{l|}{34 773} & 19 527 & \multicolumn{1}{l|}{20 214} & 16 202 & \multicolumn{1}{l|}{11 530} & 8 655 & \multicolumn{1}{l|}{4 149} & 3 688 & \multicolumn{1}{l|}{2 633} & 2 391 \\ \hline
Nb Reduc   & \multicolumn{1}{l|}{5 120}   & 3 969  & \multicolumn{1}{l|}{7 081}  & 4 879  & \multicolumn{1}{l|}{5 293}  & 3 386  & \multicolumn{1}{l|}{1 576}  & 1 291  & \multicolumn{1}{l|}{1 055}  & 998    & \multicolumn{1}{l|}{2 531}  & 1 545 & \multicolumn{1}{l|}{966}   & 812   & \multicolumn{1}{l|}{982}   & 463   \\ \hline
Nb LOOP    & \multicolumn{1}{l|}{409}     & 258    & \multicolumn{1}{l|}{818}    & 417    & \multicolumn{1}{l|}{814}    & 360    & \multicolumn{1}{l|}{341}    & 155    & \multicolumn{1}{l|}{162}    & 93     & \multicolumn{1}{l|}{415}    & 253   & \multicolumn{1}{l|}{185}   & 133   & \multicolumn{1}{l|}{160}   & 68    \\ \hline
Nb SUBSET  & \multicolumn{1}{l|}{3}       & 1      & \multicolumn{1}{l|}{2}      & 0      & \multicolumn{1}{l|}{3}      & 0      & \multicolumn{1}{l|}{3}      & 0      & \multicolumn{1}{l|}{2}      & 0      & \multicolumn{1}{l|}{4}      & 2     & \multicolumn{1}{l|}{1}     & 1     & \multicolumn{1}{l|}{1}     & 0     \\ \hline
Nb IN      & \multicolumn{1}{l|}{431}     & 495    & \multicolumn{1}{l|}{924}    & 929    & \multicolumn{1}{l|}{427}    & 433    & \multicolumn{1}{l|}{199}    & 147    & \multicolumn{1}{l|}{113}    & 113    & \multicolumn{1}{l|}{374}    & 205   & \multicolumn{1}{l|}{193}   & 160   & \multicolumn{1}{l|}{126}   & 35    \\ \hline
Nb OUT     & \multicolumn{1}{l|}{4 084}   & 3 137  & \multicolumn{1}{l|}{5 051}  & 3 487  & \multicolumn{1}{l|}{3 763}  & 2 414  & \multicolumn{1}{l|}{963}    & 961    & \multicolumn{1}{l|}{717}    & 779    & \multicolumn{1}{l|}{1 477}  & 1 082 & \multicolumn{1}{l|}{550}   & 504   & \multicolumn{1}{l|}{585}   & 360   \\ \hline
Nb PIE     & \multicolumn{1}{l|}{193}     & 78     & \multicolumn{1}{l|}{284}    & 46     & \multicolumn{1}{l|}{282}    & 179    & \multicolumn{1}{l|}{70}     & 28     & \multicolumn{1}{l|}{61}     & 13     & \multicolumn{1}{l|}{259}    & 3     & \multicolumn{1}{l|}{36}    & 14    & \multicolumn{1}{l|}{110}   & 0     \\ \hline
Nb ISOL.   & \multicolumn{1}{l|}{0}       & 0      & \multicolumn{1}{l|}{2}      & 0      & \multicolumn{1}{l|}{4}      & 0      & \multicolumn{1}{l|}{0}      & 0      & \multicolumn{1}{l|}{0}      & 0      & \multicolumn{1}{l|}{0}      & 0     & \multicolumn{1}{l|}{1}     & 0     & \multicolumn{1}{l|}{0}     & 0     \\ \hline
\end{tabular}
\end{table}


==> latex/tables/two_graph_metrics.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
               & \multicolumn{2}{c|}{WordNet}          & \multicolumn{2}{c|}{MerWeb}            & \multicolumn{2}{c|}{WEDT}              & \multicolumn{2}{c|}{LDOCE}             & \multicolumn{2}{c|}{CIDE}              & \multicolumn{2}{c|}{WCDT}            & \multicolumn{2}{c|}{WLDT}            & \multicolumn{2}{c|}{WILD}            \\ \hline
Nb vertices    & \multicolumn{1}{l|}{146 498} & 52 153 & \multicolumn{1}{l|}{97 495}  & 59 411  & \multicolumn{1}{l|}{52 565}  & 32 650  & \multicolumn{1}{l|}{35 599}  & 21 869  & \multicolumn{1}{l|}{21 095}  & 18 912  & \multicolumn{1}{l|}{12 379} & 10 620 & \multicolumn{1}{l|}{4 508}  & 4 475  & \multicolumn{1}{l|}{3 213}  & 3 064  \\ \hline
Size Kernel    & \multicolumn{1}{l|}{7 131}   & 11 277 & \multicolumn{1}{l|}{9 070}   & 13 495  & \multicolumn{1}{l|}{6 694}   & 9 148   & \multicolumn{1}{l|}{1 988}   & 3 450   & \multicolumn{1}{l|}{1 711}   & 3 602   & \multicolumn{1}{l|}{2 813}  & 3 252  & \multicolumn{1}{l|}{1 103}  & 1 451  & \multicolumn{1}{l|}{1 291}  & 1 068  \\ \hline
Size Red. Ker. & \multicolumn{1}{l|}{2 068}   & 2 948  & \multicolumn{1}{l|}{1 968}   & 2 846   & \multicolumn{1}{l|}{1 601}   & 1 836   & \multicolumn{1}{l|}{436}     & 931     & \multicolumn{1}{l|}{696}     & 1 067   & \multicolumn{1}{l|}{389}    & 374    & \multicolumn{1}{l|}{147}    & 95     & \multicolumn{1}{l|}{408}    & 216    \\ \hline
NC Red Ker.    & \multicolumn{1}{l|}{2 028}   & 2 928  & \multicolumn{1}{l|}{1 933}   & 2 807   & \multicolumn{1}{l|}{1 556}   & 1 822   & \multicolumn{1}{l|}{423}     & 915     & \multicolumn{1}{l|}{683}     & 1 058   & \multicolumn{1}{l|}{342}    & 353    & \multicolumn{1}{l|}{123}    & 85     & \multicolumn{1}{l|}{398}    & 184    \\ \hline
Init. Nb Arcs  & \multicolumn{1}{l|}{765 481} & 311321 & \multicolumn{1}{l|}{495 385} & 337 376 & \multicolumn{1}{l|}{273 432} & 190 470 & \multicolumn{1}{l|}{173 737} & 147 319 & \multicolumn{1}{l|}{107 638} & 144 308 & \multicolumn{1}{l|}{61 282} & 56 102 & \multicolumn{1}{l|}{19 133} & 21 683 & \multicolumn{1}{l|}{22 667} & 16 579 \\ \hline
Final Nb Arcs  & \multicolumn{1}{l|}{14 858}  & 32 277 & \multicolumn{1}{l|}{14 278}  & 33 268  & \multicolumn{1}{l|}{11 109}  & 19 147  & \multicolumn{1}{l|}{2 700}   & 8 943   & \multicolumn{1}{l|}{4 837}   & 11 940  & \multicolumn{1}{l|}{2 524}  & 3 665  & \multicolumn{1}{l|}{833}    & 1 149  & \multicolumn{1}{l|}{2 860}  & 1 828  \\ \hline
NC Final Arcs  & \multicolumn{1}{l|}{14 430}  & 31 766 & \multicolumn{1}{l|}{13 831}  & 32 754  & \multicolumn{1}{l|}{10 520}  & 18 849  & \multicolumn{1}{l|}{2 539}   & 8 741   & \multicolumn{1}{l|}{4 697}   & 11 660  & \multicolumn{1}{l|}{2 177}  & 3 460  & \multicolumn{1}{l|}{703}    & 1 076  & \multicolumn{1}{l|}{2 664}  & 1 424  \\ \hline
Nb Undefined   & \multicolumn{1}{l|}{144}     & 4 504  & \multicolumn{1}{l|}{328}     & 6 010   & \multicolumn{1}{l|}{89}      & 4 309   & \multicolumn{1}{l|}{46}      & 1 279   & \multicolumn{1}{l|}{22}      & 1 565   & \multicolumn{1}{l|}{48}     & 1 365  & \multicolumn{1}{l|}{33}     & 573    & \multicolumn{1}{l|}{11}     & 389    \\ \hline
Nb Undefining  & \multicolumn{1}{l|}{137 815} & 40 509 & \multicolumn{1}{l|}{86 374}  & 44 626  & \multicolumn{1}{l|}{44 280}  & 22 863  & \multicolumn{1}{l|}{33 246}  & 18 261  & \multicolumn{1}{l|}{18 843}  & 15 105  & \multicolumn{1}{l|}{9 278}  & 7 316  & \multicolumn{1}{l|}{3 261}  & 2997   & \multicolumn{1}{l|}{1 874}  & 1 991  \\ \hline
Nb SCCs Kernel & \multicolumn{1}{l|}{253}     & 81     & \multicolumn{1}{l|}{459}     & 188     & \multicolumn{1}{l|}{385}     & 112     & \multicolumn{1}{l|}{168}     & 71      & \multicolumn{1}{l|}{65}      & 23      & \multicolumn{1}{l|}{125}    & 68     & \multicolumn{1}{l|}{49}     & 27     & \multicolumn{1}{l|}{18}     & 22     \\ \hline
\end{tabular}
\end{table}

